Robustness via Uncertainty-aware Cycle Consistency

Unpaired image-to-image translation refers to learning inter-image-domain mapping without corresponding image pairs. Existing methods learn deterministic mappings without explicitly modelling the robustness to outliers or predictive uncertainty, leading to performance degradation when encountering unseen perturbations at test time. To address this, we propose a novel probabilistic method based on Uncertainty-aware Generalized Adaptive Cycle Consistency (UGAC), which models the per-pixel residual by generalized Gaussian distribution, capable of modelling heavy-tailed distributions. We compare our model with a wide variety of state-of-the-art methods on various challenging tasks including unpaired image translation of natural images, using standard datasets, spanning autonomous driving, maps, facades, and also in medical imaging domain consisting of MRI. Experimental results demonstrate that our method exhibits stronger robustness towards unseen perturbations in test data. Code is released here: https://github.com/ExplainableML/UncertaintyAwareCycleConsistency.

==> figs/translate_quality.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{pics/cityscapes_quant.png}
    \caption{
    Evaluation of different methods on Cityscapes with Gaussian perturbation under varying noise levels. NL0 denotes clean images without noise, NL1, NL2, NL3 are unseen noise levels.
    \texttt{ACC.Segm}, \texttt{IoU.Segm}, \texttt{IoU.P2P} are three metrics for evaluating translation quality. Higher is better.
    }
    \label{fig:quant_cityscapes}
\end{figure*}
